Does Momentum Change the Implicit Regularization on Separable Data?

The momentum acceleration technique is widely adopted in many optimization algorithms. However, there is no theoretical answer on how the momentum affects the generalization performance of the optimization algorithms. This paper studies this problem by analyzing the implicit regularization of momentum-based optimization. We prove that on the linear classification problem with separable data and exponential-tailed loss, gradient descent with momentum (GDM) converges to the L2 max-margin solution, which is the same as vanilla gradient descent. That means gradient descent with momentum acceleration still converges to a low-complexity model, which guarantees their generalization. We then analyze the stochastic and adaptive variants of GDM (i.e., SGDM and deterministic Adam) and show they also converge to the L2 max-margin solution. Technically, to overcome the difficulty of the error accumulation in analyzing the momentum, we construct new potential functions to analyze the gap between the model parameter and the max-margin solution. Numerical experiments are conducted and support our theoretical results.

==> Introduction_RelateWorks.tex <==
\section{Introduction}
\label{sec: intro}
\qi{The momentum acceleration technique is widely adopted in the optimization algorithms in both convex and non-convex learning tasks \cite{}. Due to its popularity in applications, there are a lot of works to study its theoretical properties. Most of the works regard on the convergence rate analysis \cite{}. However, the theoretical understanding on whether momentum influences the generalization performance of the optimization algorithms is still unclear.}

%One charming property of deep learning techniques is that they can achieve low error in both the training set and test set \citep{neyshabur2014search}. This phenomenon, however, contradicts to the landscape research of deep neural networks \citep{choromanska2015loss}, which indicates there exists numerous local minima among the parameter space while only few of them are with desired generalization properties. 

 \qi{One plausible tool to explain the generalization is to characterize the implicit bias of optimizers,} which are proposed to explore the role of optimizer in selecting the output parameters among all local minima on the landscape \citep{soudry2018implicit}. Recent efforts on analyzing the implicit bias of gradient descent (GD) and its stochastic or adaptive variants on classification problem with exponential-tailed loss have yielded many exciting developments. For instance, \cite{soudry2018implicit} pioneer the study of implicit bias of gradient descent on the linear classification task, and obtain the direction of parameters converges to the $L^2$ max margin solution; \cite{nacson2019stochastic} extend the result of \cite{soudry2018implicit} to stochastic gradient descent (SGD) by proving the same result holds almost surely;  \cite{qian2019implicit} study the same task as \citep{soudry2018implicit} with the AdaGrad optimizer, showing the convergent direction of AdaGrad depends on the optimization trajectory, and is less stable than gradient descent; \cite{lyu2019gradient} and \cite{wang2021implicit} extends the results in \citep{soudry2018implicit} and \citep{qian2019implicit} to gradient descent and adaptive optimizers for homogeneous neural networks respectively.

However, almost all existing theoretical analysis of implicit bias \qi{do not hold for optimizers with momentum}, while the default choice is momentum-based optimizers (e.g., Stochastic Gradient Descent with Momentum (SGDM) and Adaptive Momentum Estimation (Adam)) in practice \citep{vaswani2017attention,tan2019efficientnet}. A natural question is:

\centerline{\emph{Can we theoretically analyze the implicit bias of momentum-based optimizers?}}

\qidel{Specifically, it is desired to obtain the form of solution given by momentum-based optimizers satisfying (1) on classification problem with exponential-tailed loss as previous works; (2) with constant learning rate and constant momentum hyper-parameters, which are widely adopted in practice. However, under this circumstance, there is rare literature even only for the loss convergence analysis, as the loss is not monotonously decreasing any longer. To the best of our knowledge, the only related work is \citep{sun2019non}, which proves the convergence rate of gradient descent with momentum is $\mathcal{O}(t^{-1})$ (where $t$ is the iteration number). However, their result requires the loss to be coercive (i.e. loss diverges to infinity when parameters diverge to infinity), which precludes the exponential-tailed loss in the classification task; global smoothness is also required, which rules out loss functions including the exponential loss $\ell_{exp}(x)=e^{-x}$. Therefore, their analysis can not be applied to this case.} \qi{*****I suggest to put the related work \citep{sun2019non} to related works section. And move merge the introduction on the basic setting to our study, because readers may confused with the constraints on the setting. We can directly introduce our story after we ask the question.*****}

In this paper, we take the first step to analyze the convergence of momentum based optimizers \qi{****please merge the basic setting in previous paragraph here.****} \qidel{with constant learning rate and constant momentum hyper-parameters}, and obtain their implicit bias. Specifically, we study the classification problem with linear model and exponential-tailed loss using \qidel{Gradient Descent with Momentum (GDM) and} SGDM \qi{and Adam} optimizers. Our main results can be concluded as Theorem \ref{thm: inform}, which states GDM and SGDM converges to the $L^2$ max margin solution, which is the same as GD and SGD.
\begin{theorem}[informal]
\label{thm: inform}
With linear separable dataset $\bS$, for SGDM and Adam, the loss converges to $0$ with rate $\mathcal{O}(\frac{1}{t})$, the parameter norm diverges to infinity, and direction of parameters converges to the solution of the $L^2$ max margin problem ${\max}_{\bw \in \textbf{Unit}(0,1)} \min_{(\bx,\by)\in \bS} \langle \by\bx, \bw\rangle$.
\end{theorem}

Theorem \ref{thm: inform} indicates changing the gradient term in {GD} and its stochastic variant SGD into momentum will not affect the convergent direction, and the generalization behavior of the output parameters of GDM and SGDM are fairly good as the margin of a classifier is positively correlated with its generalization error \citep{jiang2019fantastic}. \qi{Please revise the optimizers.} {Moreover, our results \qidel{is} \qi{are} supported by existing experimental observations. Specifically, \citet{soudry2018implicit} observes that the GD and GDM behaves similarly in terms of convergence and margin (c.f. Figure 1, \citep{soudry2018implicit}); \citet{nacson2019stochastic} also observe this similarity between SGD and SGDM (c.f. Figure 2, \cite{nacson2019stochastic}).}

\textbf{The technical contribution} can be summarized as: (1). We propose a \emph{new Lyapunov function} to analyze the convergence of SGDM, which helps to bound the sum of squared gradients along the training trajectory; (2). We construct a new Lyapunov function to bound the difference of learned parameters and the scaled max-margin solution, which finally leads to the direction convergence. The proof techniques are general and can be applied to other analysis of momentum-based optimizers. 

\textbf{Organization of This Paper.} 
Section \ref{sec: related_work} collects further related works on the implicit bias of first order optimizers and convergence of momentum-based optimizers. Section \ref{sec: preliminary} shows basic settings and assumptions which will be used throughout this paper. Section \ref{subsec: main_gdm} studies the implicit bias of GDM as a warm up, while Section \ref{subsec: main_sgdm} and Section \ref{subsec: main_adam} explore respectively the implicit bias of SGDM and Adam. Discussions of these results are put in Section \ref{sec: discussion}.


\section{Further Related Works}
\label{sec: related_work}
\textbf{Implicit Bias of First-order Optimization Methods.} \citet{soudry2018implicit} proved that gradient descent on linear classification problem with exponential-tailed loss converges in the direction of the max $L^2$ margin solution of the corresponding hard-margin Support Vector Machine.  \citet{nacson2019stochastic} extends the results in \citep{soudry2018implicit} to the stochastic case, proving the convergent direction of SGD is the same as GD almost surely. \citet{qian2019implicit} go beyond the vanilla gradient descent methods and consider the AdaGrad optimizer instead. They prove the convergent direction of AdaGrad has a dependency in the optimizing trajectory, which varies according to initialization. \cite{ji2021characterizing} propose a primal-dual analysis framework for the linear classification models, utilizing which they provide an alternative proof of results in \citep{soudry2018implicit}, and achieve a faster convergent rate of margin by increasing the learning rate according to the loss. Based on \citep{ji2021characterizing}, \citet{ji2021fast} design another algorithm with an even faster convergent rate of margin by applying the Nesterov's Acceleration Method on the dual space. However, the corresponding form of the algorithm on the primal space is no longer a Nesterov's Acceleration Method nor GDM, which is significantly different from our settings.

On the other hand, there is another line of work trying to extend the result in the linear case to deep neural networks. \citet{ji2018gradient,gunasekar2018implicit} studied the deep linear network and \citet{soudry2018implicit} studied the two-layer neural network with ReLU activation. \citet{lyu2019gradient} propose a framework to analyze the asymptotic direction of GD on homogeneous neural networks, proving that given there eixts a time the network achieves $100\%$ training accuracy, GD will converge to some KKT point of the $L^2$ max margin problem. \citet{wang2021implicit} extends the framework of \citep{lyu2019gradient} to adaptive optimizers, and prove RMSProp and Adam without momentum have the same convergent direction as GD, while AdaGrad doesn't. The results of \citep{lyu2019gradient} and \citep{wang2021implicit} indicate results in the linear model can be extended to deep homogeneous neural networks, and suggest linear model is a proper start point to study implicit bias.

\textbf{Convergence of Momentum-Based Optimization Methods.} For convex optimization problems, the convergent rate of Nesterov's Acceleration Method has been proved once it was proposed by \citep{nesterov1983method}. By contrast, although GDM (Polyak's Heavy-Ball Method) was proposed in \citep{polyak1964some} prior to the Nesterov's Acceleration Method, the convergence of GDM on convex loss with Lipschitz gradient was not solved until \citep{ghadimi2015global} provides an ergodic convergent result for GDM (i.e., convergent result for the running average of the iterates). However, the ergodic result is undesired, as in practice, optimizing algorithms usually output the parameters of the last step. To the best of our knowledge, there are only two works on the non-ergodic analysis of GDM: \citep{sun2019non} and \cite{tao2021role}. However, \citep{sun2019non} requires the optimization target goes to infinity whenever parameter norm goes to infinity, which doesn't match the classification task adopting exponential-tailed loss (e.g., the logistic loss); \cite{tao2021role} analyzes one case with momentum hyper-parameter increasing to $1$, which contradicts to the constant momentum hyper-parameter used in practice. \cite{tao2021role} further requires the gradient is bounded all over the parameter space, which is quite restricted.

==> Tex Files/Checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~...}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section \ref{sec: intro}.}
  \item Did you describe the limitations of your work?
 \answerYes{See Section \ref{sec: discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section \ref{sec: preliminary}.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See the appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See \href{https://anonymshare.com/bbqm/main.py}{\color{blue}this link}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix \ref{appen: experiment}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We conduct the experiments across various random seeds.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{The experiments are light.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We use either synthetic data or public dataset (MNIST).}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Tex Files/MainResults.tex <==


\section{The Implicit Bias of GDM}
\label{subsec: main_gdm}
In this section, we analyze the implicit bias of GDM with a two-stage framework \footnote{It should be noticed that in the analysis of Sections \ref{subsec: main_gdm}, \ref{subsec: main_sgdm}, and \ref{subsec: main_adam}, we only prove the conclusion for almost every dataset (means except a zero-measure set in $\mathbb{R}^{d\times N}$)  for the  simplicity of illustration. However, the proof can be extended to every dataset with a more careful analysis (please refer to Appendix \ref{appen: every_data_set} for details). }. Latter, we will use this framework to further investigate SGDM and {\color{red} deterministic Adam}. The formal theorem of the implicit bias of GDM is as follows:


\begin{theorem}
\label{thm: gdm_main}
Let Assumptions \ref{assum: separable}, \ref{assum: exponential-tailed}, and \ref{assum: smooth}. (\textbf{D}) hold. Let $\beta \in [0,1)$ and $\eta<2\frac{N}{\sigma_{max}^2H_{\ell^{-1}}(N\mathcal{L}(\boldsymbol{w}_1))}$ ($\ell^{-1}$ is the inverse function of $\ell$). Then, for almost every data set $S$, with arbitrary initialization point $\bw(1)$, GDM (Eq.~\eqref{eq: def_gdm}) satisfies that
$\bw(t)-\ln(t) \hbw$ is bounded as $t\rightarrow \infty$, and $\lim_{t\rightarrow\infty}\frac{\bw(t)}{\Vert \bw(t) \Vert} =\frac{\hbw}{\Vert \hbw \Vert}$.
\end{theorem}


Theorem \ref{thm: gdm_main} adopts a constant momentum hyper-parameter, which agrees with the practical use (e.g., $\beta$ is set to be $0.9$ \cite{xie2017aggregated}). Also, Theorem \ref{thm: gdm_main} puts no restriction on the range of $\beta$, which allows wider choices of hyper-parameter tuning. Theorem \ref{thm: gdm_main} further shows that the implicit bias of GDM agrees with GD in linear classification with exponential-tailed loss (c.f. \cite{soudry2018implicit} for results on GD), and this consistency can be verified by existing and our experiments (c.f. Section \ref{sec: discussion} for detailed discussions).


We then present a proof sketch of Theorem \ref{thm: gdm_main}, which is divided into two parts: we first prove that the sum of squared gradients is bounded, which indicates both the loss and the norm of gradient converge to $0$ and the parameter diverges to infinity; these properties will then be applied to show the difference between $\bw(t)$ and $\ln(t) \hbw$ is bounded, and therefore, the direction of $\hbw$ dominates as $t\rightarrow \infty$.

\textbf{Stage I: Bound the sum of squared gradients.} The core of Stage I is to select a proper potential function $\xi(t)$, which is required to correlated with the training loss $\mL$ and be non-increasing along the optimization trajectory. For GD, since $\mL$ itself is non-increasing with properly chosen learning rate, we can just pick $\xi(t)=\mL(t)$. However, as the update of GDM doesn't align with the direction of negative gradient, training loss $\mL(t)$ in GDM is no longer monotonously decreasing, and the potential function requires special construction. Inspired by \cite{sun2019non}, we choose the following $\xi(t)$:

\begin{lemma}
\label{lem: update_rule_loss_gdm}
Let all conditions in Theorem \ref{thm: gdm_main} hold. Define $\xi(t)\overset{\triangle}{=}\mL(\bw(t))+\frac{1-\beta}{2\beta\eta} \Vert \bw(t)-\bw(t-1)\Vert^2.$  Let ${ C_1}$ be the positive real with $\eta=2\frac{N}{\sigma_{max}^2H_{\ell^{-1}}(N\mathcal{L}(\boldsymbol{w}_1))} { C_1}$. We then have  
\small
\begin{align}
\label{eq: gdm_direct_taylor}
   \xi(t)
    \ge\xi(t+1)
    +\frac{1-{ C_1}}{\eta}\Vert \bw(t+1)-\bw(t)\Vert^2.
\end{align}    \normalsize
\end{lemma}
\begin{remark}
Although this potential function is obtained by \cite{sun2019non} by directly examining the Taylor's expansion at $\bw(t)$, the proof here is non-trivial as we only requires the loss to be locally smooth instead of globally smooth in \cite{sun2019non}, and we need to prove the smoothness parameter along the trajectory is upper bounded. We defer the detailed proof to Appendix \ref{appen: gdm_sum_finite}.
\end{remark}

% To prove Lemma \ref{lem: update_rule_loss_gdm}, we define $\bw(t+\alpha)=\alpha\bw(t)+(1-\alpha)\bw(t+1)$ for any $t\in\mathbb{Z}^{+}$ and $\alpha \in (0,1)$, and prove a generalized version of Eq. (\ref{eq: gdm_direct_taylor}):
% \fontsize{8.5pt}{24pt}
% \begin{align}
% \label{eq: gdm_direct_taylor_extended}
%     \xi(t)
%     \ge \xi(t+\alpha)
%     +\frac{(1-\beta)(1-c)\alpha^2}{\eta}\Vert \bw(t+1)-\bw(t)\Vert^2.
% \end{align}
% \normalsize
%  The proof idea is that as long as Eq. (\ref{eq: gdm_direct_taylor_extended}) holds for all time in $[1,t+\alpha)$, the training loss across $[1,t+\alpha]$ will be smaller than $\mL(\bw(1))$, and the strict inequality in Eq. (\ref{eq: gdm_direct_taylor_extended}) holds. Consequently, there exists some small enough positive real $\varepsilon$, such that Eq. (\ref{eq: gdm_direct_taylor_extended}) holds for all time in $[1,t+\alpha+\varepsilon)$, and we are able to extend the feasible set where Eq. (\ref{eq: gdm_direct_taylor_extended}) holds.
%  The formal description of the generalized lemma and its corresponding proof is deferred to Appendix \ref{appen: gdm_sum_finite}.
 
 
By Lemma \ref{lem: update_rule_loss_gdm}, we have that $  \xi(t)$ is monotonously decreasing by gap $\frac{1-C_1}{\eta}\Vert \bw(t+1)-\bw(t)\Vert^2$. As $ \xi(1)=\mL(\bw(1))$ is a finite number, we have $\sum_{t=1}^{\infty}\Vert \bw(t+1)-\bw(t)\Vert^2<\infty$. One can then easily check that $\sum_{t=1}^{\infty}\Vert \nabla \mL (\bw(t))\Vert^2<\infty$ using the negativeness of the individual loss and the separability of the dataset.

% \vspace{-7pt}
%  {\color{red}The proof of Corollary \ref{lem: sum_of_squared_gradient_converge} can be found in  Appendix \ref{appen: gdm_sum_finite}. Resulted from Corollary \ref{lem: sum_of_squared_gradient_converge}, we have $ \Vert \nabla \mL(\bw(t))\Vert^2\rightarrow0$ as $t\rightarrow \infty$, which by the exponential-tailed loss assumption further leads to $\lim_{t\rightarrow \infty} \mL(\bw(t))=0$.}
 
 \textbf{Stage II. Derive the asymptotic direction.}  To derive the asymptotic direction, \cite{soudry2018implicit} and \cite{nacson2019stochastic} directly bound the norm of $\br(t)\overset{\triangle}{=}\bw(t) -\ln (t)\hbw-\tbw$, where $\tbw$ is some constant vector. Specifically, with the following simple calculation 
 \begin{equation*}
     \Vert\br(T+1)\Vert^2=\Vert\br(1)\Vert^2+2\sum_{t=1}^T \langle -\eta\nabla \mL(\bw(t))-\ln \frac{t}{t-1}\hbw, \br(t)\rangle+ \sum_{t=2}^T \Vert\eta \nabla \mL(\bw(t))-\ln \frac{t}{t-1}\hbw \Vert^2,
 \end{equation*}
 \cite{soudry2018implicit} further proves $\sum_{t=2}^T \langle -\eta\nabla \mL(\bw(t))-\ln \frac{t}{t-1}\hbw, \br(t)\rangle<\infty$ and $\br(*)$ is thus uniformly bounded. While it can be proved that $\sum_{t=2}^T \langle -\eta\nabla \mL(\bw(t))-\ln \frac{t}{t-1}, \br(t)\rangle<\infty$ still holds for GDM, the dynamic of $ \Vert\br(T+1)\Vert^2$ becomes 
  \begin{equation*}
     \Vert\br(T+1)\Vert^2=\Vert\br(1)\Vert^2+2\sum_{t=1}^T \langle \bw(t+1)-\bw(t)-\ln \frac{t+1}{t}\hbw, \br(t)\rangle+ \sum_{t=1}^T \Vert\bw(t+1)-\bw(t)-\ln \frac{t+1}{t}\hbw \Vert^2,
 \end{equation*}
 and the approach in \cite{soudry2018implicit}  cannot be directly applied here as $\bw(t+1)-\bw(t)$ now contains historical information of gradients. To handle this problem, we then analyze the following continuous dynamics approximation of GDM \cite{sun2019non} to gain intuitions:
\small
\begin{equation*}
    \frac{\beta}{1-\beta}\frac{\mathrm{d}^2 \bw(t)}{\mathrm{d} t^2}+ \frac{\mathrm{d} \bw(t)}{\mathrm{d} t}+\eta \nabla \mL(\bw(t))=0.
\end{equation*}
\normalsize
Specifically, we have
\begin{small}
 \begin{align*}
   &\frac{1}{2}\Vert\br(T)\Vert^2-\frac{1}{2}\Vert\br(1)\Vert^2=\int_{1}^T\frac{1}{2} \frac{\mathrm{d}\Vert \br(s) \Vert^2}{\mathrm{d} s} \mathrm{d} s
   \\
   =&\int_{1}^T\left\langle \br(s), - \eta\nabla \mL(\bw(s))-\frac{1}{s} \hbw\right\rangle\mathrm{d} s+\int_{1}^T\frac{\beta}{1-\beta}\left\langle \br(s), -\frac{\mathrm{d}^2 \bw(s)}{\mathrm{d} s^2}\right\rangle \mathrm{d} s,
 \end{align*}
\end{small}
and by integration by part,
\begin{small}
\begin{equation*}
    \int_{1}^T\left\langle \br(s), -\frac{\mathrm{d}^2 \bw(s)}{\mathrm{d} s^2}\right\rangle \mathrm{d} s=\left\langle \br(T), -\frac{\mathrm{d} \bw(T)}{\mathrm{d} t}\right\rangle-\left\langle \br(1), -\frac{\mathrm{d} \bw(1)}{\mathrm{d} t}\right\rangle+\int_{1}^T\left\langle  \frac{\mathrm{d} \br(s)}{\mathrm{d} s}, \frac{\mathrm{d} \bw(s)}{\mathrm{d} s}\right\rangle \mathrm{d} s.
\end{equation*}
\end{small}
As the results from Stage I and \cite{soudry2018implicit} can be interpreted in the continuous limit as $\int_{1}^\infty\langle  \frac{\mathrm{d} \bw(s)}{\mathrm{d} s},$ $ \frac{\mathrm{d} \bw(s)}{\mathrm{d} s}\rangle \mathrm{d} s<\infty$ and $\int_{1}^\infty\langle \br(s), - \eta\nabla \mL(\bw(s))-\frac{1}{s} \hbw\rangle\mathrm{d} s<\infty$, we have 
$\frac{1}{2}\Vert\br(T)\Vert^2+$ $\frac{\beta}{1-\beta}\langle \br(T), -\frac{\mathrm{d} \bw(T)}{\mathrm{d} t}\rangle$ is upper bounded, which then leads to that $\frac{1}{2}\Vert\br(T)\Vert^2$ is upper bounded as $\frac{\mathrm{d} \bw(T)}{\mathrm{d} t} \rightarrow 0$. The above methodology leads to the following claim for the discrete case (see Appendix \ref{subsubsec: form of the solution_gdm} for proofs):

\begin{claim}
\label{claim: direction_convergence}
Define potential function $g:\mathbb{Z}^{+}\rightarrow\mathbb{R}$ as 
\begin{small}
\begin{align*}
    g(t)\overset{\triangle}{=}\frac{1}{2}\Vert \br(t)\Vert^2+\frac{\beta}{1-\beta}\langle \br(t),\bw(t)-\bw(t-1)\rangle
    -\frac{\beta}{1-\beta}\sum_{\tau=2}^t\langle \br(\tau)-\br(\tau-1),\bw(\tau)-\bw(\tau-1)\rangle,
\end{align*}
\end{small}
which has the following properties:

(1). $g(t+1)-g(t)=\langle -\eta\nabla \mL(\bw(t))-\ln \frac{t+1}{t}\hbw, \br(t)\rangle$, and thus $g(t)$ is uniformly upper-bounded;\\
(2). $g(t)$ is upper-bounded iff $\br(t)$ is upper-bounded, which completes the proof.
\end{claim}
The proof can be found in Appendix \ref{subsubsec: form of the solution_gdm}. It is worth mentioning that we actually provide a more easy-to-check condition for whether $\br(t)$ is bounded, i.e., "is $g(t)$ upper bounded?". Such a condition can be generalized for other momentum-based implicit bias analysis, for example, for SGDM and deterministic Adam latter in this paper.
 
 
% The first claim in Lemma \ref{lem:gdm_r_t_bounded} provides an alternative approach to verify that $\Vert \br(t) \Vert$ is bounded, while the second claim shows this approach can be fulfilled. The motivation of this lemma is to construct an easy-to-verify criterion (i.e., $g(t)$ is upper bounded) to verify that $\Vert \br(t)\Vert$ is upper bounded. To demonstrate the intuition on the construction of $g(t)$, we consider 
%  We calculate the $\frac{1}{2}\Vert\br(t)\Vert^2-\frac{1}{2}\Vert\br(1)\Vert^2$ by applying the integral of the dynamics as
%  \begin{tiny}
%  \begin{align*}
%   &\int_{1}^t\frac{1}{2} \frac{\mathrm{d}\Vert \br(s) \Vert^2}{\mathrm{d} s} \mathrm{d} s
%   \\
%   =&\int_{1}^t\left\langle \br(s), - \frac{\eta}{1-\beta}\nabla \mL(\bw(s))-\frac{1}{s} \hbw\right\rangle\mathrm{d} s+\int_{1}^t\frac{\beta}{1-\beta}\left\langle \br(s), -\frac{\mathrm{d}^2 \bw(s)}{\mathrm{d} s^2}\right\rangle \mathrm{d} s
%     \\
%     =&\frac{\beta}{1-\beta}\left(\left\langle \br(t), -\frac{\mathrm{d} \bw(t)}{\mathrm{d} t}\right\rangle-\left\langle \br(1), -{\left.\frac{\mathrm{d} \bw({  t})}{\mathrm{d} t}\right|_{t=1}}\right\rangle+\int_{1}^t\left\langle  \frac{\mathrm{d} \br(s)}{\mathrm{d} s}, \frac{\mathrm{d} \bw(s)}{\mathrm{d} s}\right\rangle \mathrm{d} s\right)
%     \\
%     +&\int_{1}^t\left\langle \br(s), -\frac{\eta}{1-\beta} \nabla \mL(\bw(s))-\frac{1}{s} \hbw\right\rangle\mathrm{d} s,
%  \end{align*}
%  \end{tiny}
 
%  where the last equation is due to Integration by part. We denote $\tilde{g}(t)=\frac{\beta}{1-\beta}(\langle \br(t), \frac{\mathrm{d} \bw(t)}{\mathrm{d} t}\rangle-\int_{1}^t\langle  \frac{\mathrm{d} \br(s)}{\mathrm{d} s}, \frac{\mathrm{d} \bw(s)}{\mathrm{d} s}\rangle \mathrm{d} s)+\frac{1}{2}\Vert \br(t) \Vert^2$, and it can be verified the derivative of $\tilde{g}(t)$ is $\langle \br(t), - \frac{\eta}{1-\beta}\nabla \mL(\bw(t))$ $-\frac{1}{t} \hbw\rangle$. By replacing $\frac{\mathrm{d} \bw(t)}{\mathrm{d} t}$ as $ \bw(t)-\bw(t-1)$, and $\frac{\mathrm{d} \br(t)}{\mathrm{d} t}$ as $ \br(t)-\br(t-1)$ in $\tilde{g}(t)$, we obtain $g(t)$, and $g(t+1)-g(t)$ has the form $\frac{1}{2}\Vert \br(t+1)-\br(t)\Vert^2+\langle \br(t), - \frac{\eta}{1-\beta}\nabla \mL(\bw(t))-\ln\frac{t+1}{t} \hbw\rangle$, which can be analyzed following the similar routine as \cite{soudry2018implicit}. The proof of the second claim is completed.
 
%  {\color{red}On the other hand, the first claim proved by (1). $\frac{1}{2}\Vert \br(t)\Vert^2+\frac{\beta}{1-\beta}\langle \br(t),\bw(t)-\bw(t-1)\rangle$ is bounded if and only if $\Vert \br(t)\Vert$ is bounded, and (2). $\sum_{\tau=2}^{\infty}\langle \br(\tau)-\br(\tau-1),$ $\bw(\tau)-\bw(\tau-1)\rangle <\infty$, as the sum of $\Vert \bw(\tau)-\bw(\tau-1)\Vert^2$ is finite, and  $\br(\tau)-\br(\tau-1)=\bw(\tau)-\bw(\tau-1)+O(1/t)$.}
 
 

\section{Tackle the difficulty brought by random sampling}
\label{subsec: main_sgdm}
In this section, we analyze the implicit bias of SGDM. Parallel to GDM, we establish the following implicit bias result for SGDM:
\begin{theorem}
\label{thm: sgdm_main}
Let Assumption \ref{assum: separable}, \ref{assum: exponential-tailed}, and \ref{assum: smooth}. (\textbf{S}) hold. Let $\beta \in [0,1)$ and $\eta<\min\{\frac{1-\beta}{1+\frac{HN}{b\gamma^2}},  \frac{(1-\beta)^3\gamma^2b}{2H^2N\beta^2}\}$. Then, for almost every data set $S$, with arbitrary initialization point $\bw(1)$, SGDM (w/. r) satisfies
$\bw(t)-\ln(t) \hbw$ is bounded as $t\rightarrow \infty$ and $\lim_{t\rightarrow\infty}\frac{\bw(t)}{\Vert \bw(t) \Vert} =\frac{\hbw}{\Vert \hbw \Vert}$, almost surely (a.s.).
\end{theorem}
Similar to the GDM case, Theorem \ref{thm: sgdm_main} shows the implicit bias of SGDM under this setting is consistent with SGD (c.f. \cite{nacson2019stochastic} for the implicit bias of SGD). This matches the observations in practice (c.f. Section \ref{sec: discussion} for details), and is latter supported by our experiments (c.f., Appendix \ref{appen: experiment}). We further add two remarks on the learning rate upper bound and extension to SGDM (w/. r).

\begin{remark}[On the learning rate] Firstly, our learning rate upper bound $\min\{\frac{1}{\frac{\sigma^2_{max}H}{N}+\frac{\sigma^4_{max}H}{b\gamma^2}},$ $  \frac{(1-\beta)^2\gamma^2b}{2H\sigma_{max}^4\beta^2}\}$ matches the order of $H,b,\sigma_{max}$ in that of SGD $2\frac{b\gamma^2}{H\sigma^4_{max}}$ \cite{nacson2019stochastic}, and indicates our analysis is tight. Secondly, as both $\frac{1}{\frac{\sigma^2_{max}H}{N}+\frac{\sigma^4_{max}H}{b\gamma^2}}$ and $ \frac{(1-\beta)^2\gamma^2b}{2H\sigma_{max}^4\beta^2}$ are monotonously increasing with respect to batch size $b$, Theorem \ref{thm: sgdm_main} also sheds light on the learning rate tuning, i.e., the larger the batch size is, the larger the learning rate is. 

\end{remark}



\begin{remark}(On SGDM (w/o. r))
\label{remark: mini_batch SGDM}
Theorem \ref{thm: sgdm_main} can be similarly extended to SGDM (w/o. r). We defer the detailed description of the corresponding theorem together with the proof to Appendix \ref{appen: mini_SGDM}.
\end{remark}

\textbf{Proof Idea.} We highlight that \textbf{the proof of SGDM is not a trivial extension of GDM and have its own merit for other optimization analysis for SGDM}. Despite the Stage II analysis is similar, the Stage I analysis of GDM no longer work for SGDM. Specifically, in Lemma \ref{lem: update_rule_loss_gdm}, Eq. (\ref{eq: gdm_direct_taylor}) no longer holds, and thus $\xi(t)$ is no longer a potential function (even with expectation, and a detailed discussion is deferred to Appendix \ref{subsec: explanation}).  

How to find a proper potential function for SGDM? We start by examining the update rule of SGD, which only \textbf{contains the gradient information of the current step} and allows a simple potential function $\mL(\bw(t))$. Therefore, if the update rule of SGDM can also be rearranged such that only the gradient information of the current step is contained, a simple potential function could be similarly constructed. Such an intuition motivates us to rearrange the update rule of SGDM as
\begin{equation*}
    \frac{\bw(t+1)-\beta \bw(t)}{1-\beta}=\frac{\bw(t)-\beta \bw(t-1)}{1-\beta}-\eta \nabla \mL_{\bB(t)}(\bw(t)),
\end{equation*}
and by defining $\bu(t)\triangleq \frac{\bw(t)-\beta \bw(t-1)}{1-\beta}=\bw(t)+\frac{\beta}{1-\beta}(\bw(t)-\bw(t-1))$, we have $\bu(t)$ is close to $\bw(t)$ (differs by order of one-step update $\bw(t)-\bw(t-1)$), and the update rule of $\bu(t)$ only contains the current-step-gradient information $ \nabla \mL(\bw(t))$. We then select potential function as $f(\bu(t))$, and a simple Taylor's expansion directly leads to:
\begin{equation*}
    \mE[\mL(\bu(t+1))|\mF_t]\approx \mL(\bu(t))-\eta\langle \nabla \mL(\bw(t)), \nabla \mL(\bu(t)) \rangle\approx \mL(\bu(t))-\eta\Vert \nabla \mL(\bw(t))\Vert^2,
\end{equation*}
i.e., $f(\bu(t))$ is a proper potential function. We then summarize the above methodology as follows:
% \begin{lemma}
% \label{lem: alter_sgdm}
% Define $\teta\overset{\triangle}{=}\frac{\eta}{1-\beta}$
% , and $\bu(1)\overset{\triangle}{=}\bw(1)$. The update rule of SGDM (Eq. \eqref{eq: def_sgdm}) is equivalent to 
% \begin{gather}
% \nonumber
%     \bu(t+1)=-\teta\nabla \mL_{\bB(t)}(\bw(t))+\bu(t),
%     \\
% \label{eq: alter_sgdm}
%     \bw(t+1)=\beta \bw(t)+(1-\beta)\bu(t+1).
% \end{gather}
% \end{lemma}
% By a simple rearrangement of the second equation, we have $\bu(t+1)=\bw(t)+\frac{1}{1-\beta} (\bw(t+1)-\bw(t))$. As $\bw(t+1)=\bw(t)+(\bw(t+1)-\bw(t))$, $\bu(t+1)$ differs from $\bw(t+1)$ only by the different coefficient of $(\bw(t+1)-\bw(t))$. The following lemma then indicates that $\mathbb{E}\mL(\bu(t))$ is a proper selection of potential function.
\begin{lemma}
\label{lem: sgdm_loss_update}
Let all conditions in Theorem \ref{thm: sgdm_main} hold. Then, 
\begin{small}
\begin{align*}
    \mE[ \mL(\bu(t+1))]\le \mE\mL(\bu(t))-\frac{\eta}{2} \mE\Vert \nabla \mL(\bw(t)) \Vert^2
    +\frac{1-\beta}{4}\eta \left(\sum_{s=1}^{t-1} \beta^{t-1-s}\mE\left\Vert  \nabla \mL(\bw(s))\right\Vert^2\right),
\end{align*}
\end{small}
and 
\small
\begin{equation*}
    \mE[ \mL(\bu(t+1))]\le \mL(\bu(1))-\sum_{s=1}^t\frac{\eta}{4} \mE\Vert \nabla \mL(\bw(s)) \Vert^2.
\end{equation*}
\normalsize
\end{lemma}
By letting $T\rightarrow \infty$ in the second claim of Lemma \ref{lem: sgdm_loss_update}, we have $\sum_{s=1}^\infty\frac{\eta}{4} \mE\Vert \nabla \mL(\bw(s)) \Vert^2$, which is indeed what we need in Stage I.

% Lemma \ref{}The upper bound of $\mE \mL(\bu(t))$, i.e.,  $\mL(\bu(1))-\sum_{s=1}^t\frac{\teta}{4}$ $\mE\Vert \nabla \mL(\bw(s)) \Vert^2$, is monotonously decreasing by $\frac{\teta}{4} \mE\Vert \nabla \mL(\bw(t)) \Vert^2$ at step $t$, and leads to the sum of expected squared gradients being finite along the optimization trajectory.

% The proof idea of Lemma \ref{lem: sgdm_loss_update} is based on the the first order Taylor's expansion of $\mL$ at $\bw(t)$, which has the form
% \small
% \begin{align*}
%     \mathbb{E}[\mL(\bu(t+1))|\mF_t]\le&\mL(\bu(t)) -\teta\langle \nabla \mL(\bu(t)),\nabla \mL(\bw(t))\rangle
%     \\
%     +&\frac{L\teta^2}{2}\mathbb{E}[\Vert  \nabla \mL_{\bB(t)}(\bw(t)) \Vert^2|\mF_t].
% \end{align*}
% \normalsize
% As $\mL$ is $H$ smooth, we have $\nabla\mL(\bu(t))=\nabla\mL(\bw(t))+\mathcal{O}(\Vert \bu(t)-\bw(t)\Vert)$, where  $\bu(t)-\bw(t)=\frac{\beta}{1-\beta}(\bw(t)-\bw(t-1))=-\eta\frac{\beta}{1-\beta}\sum_{s=1}^{t-1}\beta^{t-1-s}\nabla\mL_{\bB(s)}(\bw(s))$ has a higher degree of $\eta$ compared to $\nabla\mL(\bw(t))$. When $\eta<\min\{\frac{1-\beta}{1+\frac{HN}{b\gamma^2}},  \frac{(1-\beta)^3\gamma^2b}{2H^2N\beta^2}\}$ , $-\langle \nabla \mL(\bu(t)),\nabla \mL(\bw(t))\rangle$ can be proved to be dominated by $-\Vert \nabla \mL(\bw(t))\Vert^2$, is strictly negative and push the loss smaller.






\section{Analyze the effect of preconditioners}
\label{subsec: main_adam}

\subsection{Implicit Bias of Deterministic Adam}
In this section, we present the implicit bias of deterministic Adam, i.e., Adam without random sampling 

\begin{theorem}
\label{thm: adam_main}
Let Assumption \ref{assum: separable}, \ref{assum: exponential-tailed}, and \ref{assum: smooth}. (\textbf{D}) hold. Let $1>\beta_2>\beta_1^4\ge 0$, and the learning rate $\eta$ is a small enough constant (The upper bound of learning rate is complex, and we defer it to Appendix \ref{subsec: choice_learning_rate}).  Then, for almost every data set $S$, with arbitrary initialization point $\bw(1)$, {\color{red} deterministic Adam} (Eq.~\eqref{eq: def_adam}) satisfies that 
$\bw(t)-\ln(t) \hbw$ is bounded as $t\rightarrow \infty$, and $\lim_{t\rightarrow\infty}\frac{\bw(t)}{\Vert \bw(t) \Vert} =\frac{\hbw}{\Vert \hbw \Vert}$.
\end{theorem}


\begin{remark}[On the $\beta_1$ and $\beta_2$ range]
Almost all existing literature assume a time-decaying hyperparameter choice of $\beta_1$ or $\beta_2$ (c.f., \cite{kingma2014adam,chen2018convergence}). On the other hand, our result proves that deterministic Adam converges with constant settings of $\beta_1$ and $\beta_2$, which agrees with the practical use.
\end{remark}

\begin{remark}[On the "Contradictory" with existing experimental results]
\cite{soudry2018implicit} observe that, on a synthetic dataset, the direction of parameter output by Adam still does not converge to the max margin direction after $2\times 10^6$ iterations (but is getting closer), while GD seems to converge to the max margin direction. This seems to contradict with Theorem \ref{thm: adam_main}. We reconduct the experiments (please refer to Appendix \ref{appen:ill} for details) and found (1). such a phenomenon occurs because a large learning rate is selected, using which GD will also stuck in a direction close to max margin direction (but not equal); (2). the constructed synthetic dataset is illed-posed, as the non-support data is larger than support data by order of magnitude (which is also rare in practice). On a well-posed dataset (data used in Figure 1 in \cite{soudry2018implicit}), we observe that both Adam and GD will converge to the max margin solution rapidly.
\end{remark}

\begin{remark}[On the proof idea] The proof of deterministic Adam is very similar to that of GDM with minor changes in potential functions. Specifically, $\xi(t)$ in Lemma \ref{lem: update_rule_loss_gdm} is changed to
\begin{small}
\begin{equation*}
    \xi(t)\triangleq\mL(\bw(t))+\frac{1}{2}\frac{1-\beta_1^{t-1}}{\eta(1-\beta_1)}\left\Vert \sqrt[4]{\varepsilon\mathds{1}_d+\hbnu(t-1)}\odot (\bw(t)-\bw(t-1))\right\Vert ^2,
\end{equation*}
\end{small}
and $g(t)$ in Claim \ref{claim: direction_convergence} is changed to
\begin{small}
\begin{align*}
   &g(t)\overset{\triangle}{=}\left\langle \br(t),(1-\beta_1^{t-1}) \sqrt{\varepsilon\mathds{1}_d+\hbnu(t-1)}\odot\left(\bw(t)-\bw(t-1)\right)\right\rangle
   \frac{\beta_1}{1-\beta_1}
   \\
   &+\frac{\sqrt{\varepsilon}}{2}\Vert \br(t)\Vert^2-\frac{\beta_1}{1-\beta_1}\sum_{\tau=2}^t\langle \br(\tau)-\br(\tau-1),(1-\beta_1^{\tau-1}) \sqrt{\varepsilon\mathds{1}_d+\hbnu(\tau-1)}\odot\left(\bw(\tau)-\bw(\tau-1)\right)\rangle.
\end{align*}
\end{small}
The rest of the proof then flows similarly as the GDM case and is deferred to Appendix \ref{subsec: implicit_bias_adam}.
\end{remark}

\subsection{What if random sampling is added?}
\label{randomsam}
Till now, we have obtained the implicit bias for GDM, SGDM and {\color{red} deterministic Adam}, one may wonder whether the implicit bias of stochastic Adam can be obtained. Unfortunately, the gap can not be closed yet. The reason is that to derive the implicit bias of one desired algorithm, we first need to prove that the loss converges (specifically, the sum of squared gradient along the trajectory is finite, e.g., Corollary \ref{lem: sum_of_squared_gradient_converge}, Lemma \ref{lem: sgdm_loss_update}, and Lemma \ref{lem: adam_asymptotic}). However, deriving such a result is technically difficult even for stochastic RMSProp (i.e., Adam with $\beta_1=0$ in Eq. (\ref{eq: def_adam})) with constant learning rates. Specifically, the main difficulty lies in bounding the change of conditioner $\frac{1}{\sqrt{\varepsilon\mathds{1}_d+\hbnu(t)}}$ across iterations, which is required to make the drift term $\langle \nabla \mL(\bw(Kt)), \bw(K(t+1))-\bw(Kt)\rangle$ (derived by Taylor's expansion of the epoch start from $Kt$) large enough in absolute value for loss update. 

On the other hand, if we adopt decaying learning rates $\eta_t=\frac{1}{\sqrt{t}}$, \cite{shi2021rmsprop} shows $\beta_2$ close enough to $1$, the following equation holds for stochastic RMSProp (w/o. r) (recall that $K\triangleq\frac{N}{b}$ is the length of one epoch)
\small
\begin{equation}
\label{eq: shi_main}
    \sum_{t=0}^T \frac{1}{\sqrt{t+1}}\left\Vert \nabla \mL\left(\bw\left(Kt\right)\right)\right\Vert=\mathcal{O}(\ln T).
\end{equation}
\normalsize

Based on this result, we have the following theorem for stochastic RMSProp (w/o. r):
\begin{theorem}
\label{thm: ib_rms}
Let Assumptions \ref{assum: separable}, \ref{assum: exponential-tailed}, and \ref{assum: smooth}. (S) hold. Let $\beta_2$ be close enough to $1$.
Then for
almost every data set $S$, with arbitrary initialization point
$\bw(1)$, we have stochastic RMSProp (w/o. r) converges to the $L^2$ max margin solution.
\end{theorem}

\begin{remark}
The decaying learning rate is a "stronger" setting compared to constant learning rate, both in the sense that GDM, SGDM, and {\color{red} deterministic Adam} can be shown to converge to the max margin solution following the same routine as Theorems \ref{thm: gdm_main}, \ref{thm: sgdm_main}, and \ref{thm: adam_main}, and in the sense that we usually adopt constant learning rate in practice.
\end{remark}

The proof is on the grounds of a novel characterization of the loss convergence rate deriving from Eq. (\ref{eq: shi_main}) and the detail can be found in Appendix \ref{appen: random_shuffling_rmsprop}. 
Furthermore, the proof can be easily extended to the Stochastic Adaptive Heavy Ball (SAHB) algorithm  (proposed by \cite{tao2021role}), which can be viewed as a momentum version of RMSProp (but different from Adam) with the following update rule
\small
\begin{equation*}
    \bw(t+1)=\bw(t)-\eta_t\frac{\nabla \mL_{\bB(t)}(\bw(t))}{\sqrt{\varepsilon \mathds{1}_d+\hbnu (t)}}+\beta_1(\bw(t)-\bw(t-1)), t\ge 1.
\end{equation*}
\normalsize

The proof of Theorem \ref{thm: ib_rms} can be easily extended to SAHB, based on the fact that $\bu(t)=\frac{\bw(t)-\beta_1\bw(t-1)}{1-\beta}$ has a simple update, i.e.,
\small
\begin{gather*}
\nonumber
    \bu(t+1)=-\frac{\eta}{1-\beta_1}\frac{\nabla \mL_{\bB(t)}(\bw(t))}{\sqrt{\varepsilon \mathds{1}_d+\hbnu (t)}}+\bu(t),
\end{gather*}  
\normalsize
and $f(\bu(t))$ can be used as a potential function just as the SGDM case.
\begin{figure}[htbp]
\centering
\vspace{-1mm}


\begin{minipage}{1.0\textwidth}
\centering
\begin{subfigure}{.45\textwidth}
          \centering
          \includegraphics[width=1.0\textwidth]{Figures/Acc_main_text.png}
          \caption{Training Accuracy}
        \end{subfigure}%
        \hspace{0.4mm}
\begin{subfigure}{.45\textwidth}
          \centering
          \includegraphics[width=1.0\textwidth]{Figures/Angle_main_text.png}
          \caption{Angle gap between the parameter direction and the max margin solution}
\end{subfigure}%
\end{minipage}%
\centering
\caption{Comparison of the implicit bias of (S)GD, (S)GDM, deterministic Adam and stochastic RMSProp. We use the synthetic dataset in \cite{soudry2018implicit} with learning rate $0.1$. Figure (b) shows (1). all the optimizers converge to the max margin solution, and (2). the asymptotic behaviors with \& without momentum are similar. The experimental observation support our theoretical results.}
\label{fig: main_text}
\end{figure}

\section{Discussions}
\label{sec: discussion}


\textbf{Consistency with the Experimental Results.} We conduct experiments to verify our theoretical findings. Specifically, we (1). run GD, GDM, SGD, SGDM, and Adam on synthetic dataset to observe their implicit bias; (2). run GD and Adam on ill-posed dataset proposed in \cite{soudry2018implicit} to verify Theorem \ref{thm: adam_main}; (3). run SGD and SGDM on neural networks to classify MNIST dataset to compare their implicit regularization.  The experimental results stand with experimental observations. Furthermore, it is worth mentioning that experimental phenomenons that adding momentum will not change the implicit bias have also been observed by existing literature \cite{soudry2018implicit,nacson2019convergence,wang2021implicit}. 

\textbf{Influence of hyperparameters on convergence rates.} Our results can be further extended to provide a precise characterization on the influence of the hyperparameters $\eta$ and $\beta$ on the convergence rate of (S)GDM. Specifically, in Appendix \ref{appen: precise}, we show that the asymptotic convergence rate of (S)GDM is $C\frac{1}{\eta}\frac{1}{t}$, where $C$ is some constant independent of $\beta$ and $\eta$. Therefore, increase $\eta$ can lead to a faster convergence rate (with learning rate requirements in Theorems \ref{thm: gdm_main} and \ref{thm: sgdm_main} satisfied). However, changing $\beta$ doesn't affect the convergence rate, which is verified by our experiments (e.g. Figure \ref{fig: main_text}). This seems to be weird, as in deep learning, replacing gradient by momentum often accelerates the training. We hypothesize such an acceleration appears as the landscape of neural networks are highly non-convex and thus can not be observed in the case considered by this paper. 


\textbf{Gap Between The Linear Model and Deep Neural Networks.} While our results only hold for the linear classification problem, extending the results to the deep neural networks is possible. Specifically, existing literature \cite{lyu2019gradient,wang2021implicit} provide a framework for deriving implicit bias for deep homogeneous neural networks. It remains an interesting work to see whether our results can be constructed for GDM
and Adam for deep neural networks.

